SlackQ : Approaching the Qubit Mapping Problem with A Slack-aware Swap Insertion Scheme

The rapid progress of physical implementation of quantum computers paved the way for the design of tools to help users write quantum programs for any given quantum device. The physical constraints inherent in current NISQ architectures prevent most quantum algorithms from being directly executed on quantum devices. To enable two-qubit gates in the algorithm, existing works focus on inserting SWAP gates to dynamically remap logical qubits to physical qubits. However, their schemes lack consideration of the execution time of generated quantum circuits. In this work, we propose a slack-aware SWAP insertion scheme for the qubit mapping problem in the NISQ era. Our experiments show performance improvement by up to 2.36X at maximum, by 1.62X on average, over 106 representative benchmarks from RevLib, IBM Qiskit , and ScaffCC.

==> backup_propose.tex <==
\section{Proposed Solution}

A good way to search for the set of SWAPs that minimizes the total circuit depth is to think of how to overlap SWAPs insertions with existing gates.

Here we talks about our depth-aware SWAP insertion algorithm in this section.
\subsection{Layer Partitioning}

\begin{figure}[!ht]
  \centering
  \includegraphics[width=0.7\linewidth]{figs/layers.png}
  \caption{An example of layer partitioning }
  \label{fig:layers}
\end{figure}

First step is to partition the circuit into layers.
A layer includes all the gates that can process in parallel at a certain time. Here's an example (Fig. \ref{fig:layers}) showing how to partition the circuit into layers. A circuit of 4 CNOT gates and 6 H gates is partitioned into 5 layers, each layer has the gates that operate on independent qubits. Any gates depending on certain gate of one layer will have to be put in the following layers. The number of the layers equals the depth of the circuit. 

\subsection{Search for SWAP operations between layers}
Qubit mapping conflicts may arise between one layer and its next layer. To resolve this, we need to insert SWAPs between any two consecutive conflicting layers. We utilize the $A^{\ast}$ algorithm (shown in Fig. \ref{fig:astar}) from \cite{Zulehner+:DATE18} to search for the valid SWAPs set between layers. 


\begin{figure}[!ht]
  \centering
  \includegraphics[width=1\linewidth]{figs/astar.png}
  \caption{Overview of the $A^{\ast}$ searching algorithm}
  \label{fig:astar}
\end{figure}



For example, to find the SWAPs between layers $L_{x}$ and $L_{x+1}$, the $A^{\ast}$ algorithm starts searching from the mapping of $L_{x}$, which we call $\sigma_{0}$. From $\sigma_{0}$, the algorithm tries to insert concurrent SWAPS, and it will produce successor mappings from different number of SWAPs. If for current mapping, it can only insert $n$ concurrent SWAPs at most. The successors would be the resulting successors of 1 SWAP, 2 SWAPs and so on till n SWAPs. All these successors would be ranked based on their cost (by putting into a priority queue), which is based on inherent cost and heuristic cost. If there are successors that fulfils the CNOT constraint of the following layer $L_{x+1}$, the search is ended and the CNOT-compliant successor with the least cost would be returned. If there are no CNOT-compliant successors, the search continues and the successor with least cost is spanned such that all its successors are added to the priority queue. The algorithm keeps the process until one CNOT-compliant successor is returned. 

\subsection{Choose the SWAP layer based on critical path}
This sections talks about how we make the algorithm more depth-aware. For the $A_{\ast}$ searching, it can find more than one CNOT-compliant mapping. We then evaluate all these CNOT-compliant candidates by adding it into the current circuit and calculate the resulting depth. It turns out the one with the least cost based on the heuristic normally does not result into smallest depth. We then choose the candidate that has the smallest depth as the one CNOT-compliant successor and return it. Algorithm \ref{algo} shows the details of how it works.

\begin{figure}[!ht]
  \centering
  \includegraphics[width=1\linewidth]{figs/algo.png}
  \caption{Choose the SWAP layer based on critical path}
  \label{fig:algo}
\end{figure}

\begin{algorithm}[h!t]
\label{algo}
\SetAlgoLined
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Input{Good Mapping Candidate G }
\Output{Best Mapping with the Least Circuit Depth}
\BlankLine

 best\_mapping = $\varnothing$\;
 critical\_path\_of\_best\_mapping = $\infty$\;
 \For{x $\in$ G}{
    new\_circuit = construct\_new\_circuit(original\_circuit, x)\;
    temp\_cp = calculate\_critical\_path(new\_circuit)\;
    \If{temp\_cp $<$ critical\_path\_of\_best\_mapping }{
        critical\_path\_of\_best\_mapping = temp\_cp\;
        best\_mapping = x\;
    }
 }
 
 \caption{Depth-aware SWAP Insertion}
\end{algorithm}



\subsection{Optimizations}

\subsection{Sensitivity Study}
\begin{figure}[htb]
  \centering
  \includegraphics[width=1\linewidth]{figs/sensitivity.png}
  \caption{Sensitivity to parameters}
  \label{fig:sensitivity}
\end{figure}
We use two parameters to tune our experiment: one is denoted as "expand" which means the number of nodes to expand at the each step of the search, and another one is denoted as "deeper" which means the number of deeper levels to go down after the search found the first CNOT-compliant mapping. These two parameters can go from 1 to larger numbers. By tuning these two parameters, we gradually yield the best results for our benchmarks. As we can see in Fig. \ref{fig:sensitivity}, with increasing these two parameters, there are more benchmarks achieve better performances. This shows that if we expand more nodes in the search and increase the search depth, there could be more better solutions found. It tells us that current heuristic-based qubit mapping solutions are still far from being optimal. 

==> propose.tex <==
\section{Insight and Design}

\subsection{Metric}
As our work is a depth-aware SWAP insertion scheme, we first precisely define the metric for characterizing the depth of a circuit. In order to fully explain the metric, we need to introduce the concepts of \emph{dependency graph} and \emph{critical path}. 

The dependency graph represents the precedence relation between quantum gates in a logical quantum circuit. The definition is below:

\begin{definition}{Dependency Graph} :
The dependency graph of a quantum circuit $C$ with a set of gates $\Psi$ is a Directed Acyclic Graph $G_\psi=(\Psi, E_\psi)$, $E_\psi \subseteq \psi \times \psi$. A directed edge from node $\psi_1$ to node $\psi_2$ exists if and only if the output of gate $\psi_1$ is (part of) the input of gate $\psi_2$ in the quantum circuit $C$.
\end{definition}

The critical path is referred to as the longest path in the dependency graph. And the definition is below:


\begin{definition}{Critical Path} :
Given a dependency graph $G_\psi=(\Psi, E_\psi)$ of a quantum circuit. The critical path is $CP=Max(Path(\psi_1, \psi_2))$ $ s.t.$ $\psi_1, \psi_2 \in E_{\psi}$ $and$ $ \psi_1 \neq \psi_2$ 
\end{definition}


The depth is characterizing the number of execution steps of a quantum circuit, which is tantamount to the critical path length of the circuit. The longest path in the dependence graph describes the minimal number of steps the circuit needs in order for every gate's data dependence be resolved. In Algorithm \ref{algo}, we show how we calculate the critical path.
\begin{algorithm}[htb]
\label{algo}
\SetAlgoLined
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Input{The circuit's dependency graph $G(V,E)$ }
\Output{The critical path $CP$}
\BlankLine

%  best\_mapping = $\varnothing$\;
%  critical\_path\_of\_best\_mapping = $\infty$\;

 earliest\_start = \{\}\;
 CP = 0\;
 
 
 \For{n $\in$ V in topological order}{
    temp = 0\;
    \For{p $\in$ V's predecessors} {
      \If {temp $<$ earliest\_start[p] + latency[p]}{
         temp = earliest\_start[p] + latency[p]\;
      } 
    }
    earliest\_start[n] = temp\;
      \If {CP $<$ temp + latency[n]} {
         CP = temp\;
      }
 }
 
 
 
return CP \;
 
 \caption{Calculate the Critical Path of a Circuit}
\end{algorithm}


We first sort the nodes in the directed acyclic graph in topological order. Then we process the nodes in that order. For each node, we check the earliest start time for each of its predecessors, and add it by the latency of that predecessor, then we choose the maximum and use it as the earliest start time of this node. The maximum of all nodes' earliest start time added by their latency is the critical path length. 

We use the critical path length as the metric for ranking different swap insertion options.




% The circuit is comprised of quantum gates applied on qubits in a time order, which means a dependency tree for quantum gates can be built based on their order applied on each qubit. The critical path of this dependency tree is equal to the depth of the entire circuit. For adding SWAP into the circuit, if it's not on the critical path it is possible the result depth would not be increased. A clear example is shown in Fig. \ref{fig:simple_exp} (d), where the inserted two SWAPs render no depth increase to the circuit. In this sense, the added SWAPs overlap 100\% with existing circuit. 

% A na\"ive way towards realizing the need to overlap with the circuit, is to maximally overlap the inserted SWAPs with the already processed part of the circuit. At the certain point of needing to insert SWAPs, what we have is the already processed part of the circuit, but the remaining is still untouched. It naturally leads to the goal of merging SWAPs with existing circuit. But normally the case is that there is actually not enough potential to overlap with the previous part of the circuit. This example here clearly shows that in Fig. \ref{fig:remainingcircuit}, there is also potential to explore in the remaining circuit.

% This marks our insight that, when choosing the candidates of a SWAP set, it's ideal to consider its potential to overlap with not the existing processed circuit but the entire circuit from beginning to the end.

\subsection{Framework Design}
With the metric precisely explained in previous section, now we continue to explain the work flow of our framework and the intuitions behind it.

Before delving into the details of this framework, we need to define the \emph{layer} and the \emph{coupling graph}.

\begin{figure}[htb]
  \centering
  \includegraphics[width=0.9\linewidth]{figs/framework.pdf}
  \caption{The Qubit Mapping Framework}
  \label{fig:workflow}
\end{figure} 


\begin{definition}{Coupling Graph} : 
The coupling graph of a quantum architecture $X$ with a set of physical qubits $Q$ is a directed graph $G=(Q, E)$, $E\subseteq Q\times Q$. The edge $E_{x}=(Q_1,Q_2)\in E$ if and only if a $CNOT$ gate can be applied to $Q_1$ and $Q_2$ in $X$ with $Q_1$ being the control qubit and $Q_2$ being the target qubit. 
\end{definition}

We can divide the set of quantum gates in a circuit into layers, so that all gates in the same layer can be executed concurrently. The formal definition of a layer is:

\begin{definition}{Layer} :
A quantum circuit $C$ can be divided into layers $L = 
{l_1,l_2,l_3,...,l_m}$, while $\bigcup_{i=1}^{m}l_i = C$ and $\bigcap_{i=1}^{m}l_i = \emptyset$. The set of gates at layer $l_i$ can run concurrently  and  act on distinct sets of qubits.
\end{definition}
To divide a circuit into layers, we group the gates that have the same \emph{earliest start time} (defined in Algorithm \ref{algo}) into the same layer. The order of the layers is thus determined by the order of the \emph{earliest start times}.   

We use an iterative process to find the mapping. Our framework is depicted in Fig. \ref{fig:workflow}. And this iterative process is explained as below.
We start the framework by taking the input of the coupling graph (also denoted as \emph{Qubit Connectivity}) and the original circuit's initial layer. 

We process the circuit layer by layer. Given a layer, we perform the following steps.
    \begin{itemize}
        \item We check the layer to see if it is hardware-compliant based on the coupling graph and the qubit mapping before current layer is scheduled.
        \item If YES, we move on to next layer.
        \item If NO, we invoke our mapping searcher to search for (the set of) swaps that are necessary to solve the current layer. We consider depth-awareness during the selection of the set of swap gates -- the resulted mapping of which generates the smallest critical path length (described in Section \ref{sec:map}). After we find a hardware-compliant mapping, we move to the next layer. 
    \end{itemize}
    
    After all layers are processed, the mapping terminates. 

\subsection{Circuit Mapping Searcher}
\label{sec:map}
Here we describe the specific mapping searcher we use to overcome the coupling constraint for a given layer. 

We build our method upon the 
\emph{A-star} algorithm for finding valid mappings that minimize the number of only the inserted SWAP gates \cite{Zulehner+:DATE18}. We extend it by changing the ranking metric and allowing it to search for feasible mappings that do not necessarily have the smallest SWAP gate counts. It will help us search in a way that minimizes the depth while not significantly increasing the gate count.


%To be depth-aware for the searching process, it is important how we take the focus of depth into consideration. Thus the goal of searching becomes to find the mapping that minimizes the resulting depth while also reducing increased gate count as few as possible. 

We rank the swap options by the increase in the critical path length. Since it is an iterative process that handles the gates layer by layer, it is tempting to consider only minimizing the depth of the already processed circuit when deciding which swaps to use.  

\begin{figure}[htb]
  \centering
  \includegraphics[width=0.9\linewidth]{figs/frainsight.pdf}
  \caption{(a) Layout of an example architecture with 4 physical qubits (b) Example of a quantum circuit, the dashed line separates the processed circuit and the remaining circuit (c) Inserted SWAP overlaps with remaining circuit instead of existing processed circuit}
  \label{fig:remainingcircuit}
\end{figure} 

But the example in Fig. \ref{fig:remainingcircuit} shows that not only the processed circuit, but also the remaining circuit can help overlap the SWAPs with existing gates in the circuit without affecting the critical path.  As shown in Fig. \ref{fig:remainingcircuit}, for the CNOT gate (in red), there is no way it can overlap the necessary SWAPs with the processed circuit (dubbed as the circuit before the dashed line). But when we look after the dashed line, the three single-qubit gates can overlap with inserted SWAP. And this renders less impact to the depth of the resulting circuit, compared to if we insert the SWAP on $Q_1$ and $Q_2$.

Based on this intuition, we design our scheme of choosing the SWAP candidate as in Fig. \ref{fig:algo}. For each of the hardware-compliant remapping candidates that we acquire from the \emph{A-star} searcher, we calculate the critical path after merging the candidate (set of) swap(s) with both the processed circuit and the not-processed circuit. We choose the mapping that yields the shortest critical path.

\begin{figure}[!ht]
  \centering
  \includegraphics[width=1\linewidth]{figs/fraidea.pdf}
  \caption{Choose SWAP Candidates}
  \label{fig:algo}
\end{figure}


% \begin{figure}[!ht]
%   \centering
%   \includegraphics[width=1\linewidth]{figs/astar.png}
%   \caption{Overview of the $A^{\ast}$ searching}
%   \label{fig:astar}
% \end{figure}

% As shown in Fig. \ref{fig:astar}, the $A^{\ast}$ algorithm starts searching from current mapping. From current, the algorithm tries to insert concurrent SWAPS, and it will produce successor mappings from different number of SWAPs. If for current mapping, it can only insert $n$ concurrent SWAPs at most. The successors would be the resulting successors of 1 SWAP, 2 SWAPs and so on till n SWAPs. All these successors would be ranked based on their cost (by putting into a priority queue), which is based on inherent cost and heuristic cost. If there are successors that fulfils the CNOT constraint of the following circuit, the search is ended and the CNOT-compliant successor with the least cost would be returned. If there are no CNOT-compliant successors, the search continues and the successor with least cost is spanned such that all its successors are added to the priority queue. The algorithm keeps the process until one CNOT-compliant successor is returned. 

\subsection{Optimizations}
% The search for SWAPs start from the current mapping that needs change. And during the search process in the $A^{\ast}$ algorithm, each node inside the search tree represents a temporary mapping. 

% For the $A^{\ast}$ searching, it can find more than one CNOT-compliant mapping. We then evaluate all these CNOT-compliant candidates by adding it into the current circuit and calculate the resulting depth. It turns out the one with the least cost based on the heuristic normally does not result into smallest depth. We then choose the candidate that has the smallest depth as the one CNOT-compliant successor and return it.


We use two ways to optimize our proposed solution. One is to expand more nodes during the \emph{A-star} search, and another one is to search into deeper levels.
\subsubsection{Expand More Nodes}
In the search process for \emph{A-star}, the normal routine is to expand the one node of least cost at each step. Here, we can expand more than one node at each step and increase the search space. The number of nodes that can be expanded at a time can go from 1 to larger number. 
%In our experiments, we choose to expand 5 at one step.  
\subsubsection{Deeper Search}
 We increase the depth of the A-star search tree. In normal case, the search process ends when it finds the first node that minimizes the number of SWAPs, which is reflected as a certain level of the A-star tree. To this end, the second optimization that we applied here is to continue the search into a deeper level of the A-star tree. We can specify and tune the parameter of the deeper search. %This number can be tuned. %and we set this parameter to 4 in this paper. 

By tuning these parameters, there are more possible nodes added into our search space. With a larger search space, we have a larger possibility to jump out of one local optima and go to the global optima.


==> slackq - arxiv/background.tex <==
\section{Background and Motivation}
\label{sec:motiv}
\subsection{Quantum Computing Basics}





\subsubsection{Qubit}
A quantum bit or qubit, is the counterpart to a classical bit in the realm of
quantum computing. Different from a classical bit that represents either `1' or
`0', a qubit is in the coherent superposition of both states. The state |$\psi$> associated with a qubit is a unit vector in a two-dimensional vector space. The state of a qubit can be represented as
\begin{gather*}
 |\psi> ~ = \alpha |0> + ~\beta |1> ~= 
  \begin{bmatrix}
   \alpha \\
   \beta 
   \end{bmatrix},
\end{gather*}
where $\alpha$ and $\beta$ are two complex numbers such that $|\alpha|^2 + |\beta|^2 = 1$. $\alpha$ and $\beta$ are called amplitudes. Upon the standard measurement, the state |$\psi$> will collapse into the basis state |0> with probability $|\alpha|^2$ or 
the basis state |1> with probability $|\beta|^2$. A system of n qubits encodes a state superposition of $2^n$ basis vectors with $2^n$ amplitudes. The classical n-bit system encodes the information of one basis vector in the vector space, but n-qubit system encode the information of $2^n$-dimensional vector space. Operating on one n-qubit state is as if operating on $2^n$ complex numbers at one time. This is one of the reasons for the potential  exponential speedup using quantum computing. 

\subsubsection{Quantum Gates}
There are two types of elementary quantum gates. One is the single-qubit gate, which is a unitary quantum operation that can be abstracted as the
rotation around the axis of the Bloch sphere \cite{Nielsen+:2002book}. 
A single-qubit gate can also be represented using a 2 by 2 unitary matrix. Important single-qubit gates include the H (Hadamard) gate, and the S (phase shift by $\pi/4$)
gate \cite{amy+:tcads13}. 

The second type of gate is the multi-qubit gate. The controlled-NOT (CNOT) is a two-qubit gate that performs the most important role (arguably) in quantum computation. The two qubits involved in a CNOT gate are: the control qubit and the target qubit. If the control qubit is 0, it leaves the target qubit unchanged. If it is 1, it applies a NOT gate to the target qubit. The CNOT gate entangles qubits and allow qubits to communicate. The CNOT gate, \textsf{H} gate, \textsf{S} gate, and \textsf{T} gate together form a universal set called the \textsf{Clifford+T} library. Any quantum algorithm can be implemented using a composition of gates from the universal set.    


\subsubsection{Quantum Circuit}
A quantum algorithm can be expressed as a quantum circuit which is composed of a set of qubits and a sequence of quantum
operations on these qubits. A quantum circuit can be thought of a quantum algorithm in ``assembly language''.  There are two different ways to describe the quantum
circuits. One way is to use the quantum assembly language called
OpenQASM~\cite{Andrew+:arxiv17} released by IBM. The other way is to use a
circuit diagram, in which qubits are represented as horizontal lines. Input is the on the left and output is on the right. Unlike a classical circuit, a quantum circuit must have the same number of input and output qubits. Fig. \ref{fig:motivation}
(b) shows an example quantum circuit diagram. Logical qubits are denoted using lowercase letters (q1, q2, ...) and physical qubits are denoted using uppercase letters (Q1, Q2, ...). Initially, logical qubits q1, q2, q3, q4, and q5 are mapped to physical qubits Q1, Q2, Q3, Q4, and Q5. A single-qubit gate is denoted
as a square on the line. A CNOT gate is represented as a line connecting
two qubits where the control qubit is marked with a dot and the target qubit with a $\oplus$ sign. In this paper, we use the circuit diagram representation to describe examples. 





\subsection{Qubit Mapping Problem}
To enable the execution of a quantum circuit, the logical qubits in the circuit must be mapped to the physical qubit on the target hardware. When applying a CNOT gate, the two logical qubits involved in
the CNOT gate must be mapped to two physical qubits connected to each other. Due to the irregular layout and connectivity of the qubits in the target device, it is sometimes impossible to find an initial mapping that makes the entire circuit CNOT-compliant. The common practice is to insert SWAP operations to remap the logical qubits, whenever a CNOT gate cannot be applied. 



A SWAP operation exchanges the states of the
two input qubits of interest. As shown in Fig. \ref{fig:swapgate} (b), a swap
operation is implemented using 3 CNOT gates for architectures with
bi-directional links, where a bi-directional link means both ends of the
link can be the control or target qubit. Or it can be implemented using 3 CNOT gates plus 4 Hadamard gates for architectures
with single-direction links as shown in Fig. \ref{fig:swapgate} (c), where a single-direction link means
only one end of the link can be the control qubit.  



The qubit mapping problem takes a logical circuit and a hardware coupling graph as input and outputs a transformed circuit that fits on the hardware device by inserting SWAP operations. After the transformation, all CNOT gates must be performed on qubits that are connected in the physical architecture.  Due to the swaps, a logical qubit may be mapped to different physical qubits at different points in the circuit execution. But, at any given point, a logical qubit will be mapped to exactly one physical qubit since we are only using swaps to move qubits and are not making any copies. 
 
 \begin{figure}[!htb]
  \centering
  \includegraphics[width=1.0\linewidth]{figs/swap.pdf}
  \caption{Implementation of a SWAP operation: (a) the SWAP notation, where m and n are two logical qubits, after SWAP, m and n exchanged their states, (b) for bidirectional links, where the three CNOT that implement the SWP do not need to use the same control qubit, and (c) for single direction links, where the three CNOT must use the same control qubit.}
  \label{fig:swapgate}
\end{figure} 



An example of circuit transformation is shown in Fig. \ref{fig:motivation} where (a) is the physical connectivity, (b) is the original circuit, (c) and (d) offer two different hardware-compliant circuits generated from the same original circuit. 





\subsection{Parallelism in Quantum Circuit}
Like in classical computers, parallelism is also important in quantum computers. Parallelism comes from independent operations on different qubits. Gates on the same qubit have to run sequentially. For instance, if $a$ and $b$ are two consecutive gates on the same qubit, and $a$ is before $b$ in the program, then gate $b$ depends on $a$. Gates that do not share any qubit are independent. A two-qubit gate depend on up to two gates since it involves two qubits. A two-qubit gate has up to two immediate successors in the dependence graph. A dependence graph can be built with respect to the partial order between gates. It is a directed acyclic graph (DAG).

%as the edges have directions and there are no cycles in the graph. 

In a transformed circuit, the parallelism could be (1) between the gates in the original circuit (as \textsf{g2} and \textsf{g3} in Fig. \ref{fig:motivation} (b)), (2) between the SWAP gates that are inserted into the original circuit, and (3) between a gate in the original circuit and a newly inserted gate (as \textsf{swap 3,5} and g1 in Fig. \ref{fig:motivation}(c)). A good qubit mapping algorithm should consider all types of parallelism. However, existing studies only consider the first two types of parallelism. Our work is the first one that systematically exploits all type of parallelism. 
%and builds a formal model for the overall performance of the transformed circuit.

As shown in Fig. \ref{fig:motivation}, the best two known approaches by Zulehner \etal
\cite{Zulehner+:DATE18} and Li \etal \cite{Li+:ASPLOS19} do not distinguish solution (c) from solution (d) as the two solutions both 
insert 1 SWAP. And \cite{Zulehner+:DATE18} and \cite{Li+:ASPLOS19} only optimize the number of gates inserted into the
circuit (or the parallelism of the inserted gates), but not the parallelism of the
transformed circuit. The solution in Fig. \ref{fig:motivation} (c) is better than Fig.  \ref{fig:motivation} (d) as the inserted swap can run in parallel with the gates in the original circuit. This example stresses the importance of
time-awareness in SWAP insertion schemes and motivates our work. 




==> slackq - arxiv/backup_propose.tex <==
\section{Proposed Solution}

A good way to search for the set of SWAPs that minimizes the total circuit depth is to think of how to overlap SWAPs insertions with existing gates.

Here we talks about our depth-aware SWAP insertion algorithm in this section.
\subsection{Layer Partitioning}

\begin{figure}[!ht]
  \centering
  \includegraphics[width=0.7\linewidth]{figs/layers.png}
  \caption{An example of layer partitioning }
  \label{fig:layers}
\end{figure}

First step is to partition the circuit into layers.
A layer includes all the gates that can process in parallel at a certain time. Here's an example (Fig. \ref{fig:layers}) showing how to partition the circuit into layers. A circuit of 4 CNOT gates and 6 H gates is partitioned into 5 layers, each layer has the gates that operate on independent qubits. Any gates depending on certain gate of one layer will have to be put in the following layers. The number of the layers equals the depth of the circuit. 

\subsection{Search for SWAP operations between layers}
Qubit mapping conflicts may arise between one layer and its next layer. To resolve this, we need to insert SWAPs between any two consecutive conflicting layers. We utilize the $A^{\ast}$ algorithm (shown in Fig. \ref{fig:astar}) from \cite{Zulehner+:DATE18} to search for the valid SWAPs set between layers. 


\begin{figure}[!ht]
  \centering
  \includegraphics[width=1\linewidth]{figs/astar.png}
  \caption{Overview of the $A^{\ast}$ searching algorithm}
  \label{fig:astar}
\end{figure}



For example, to find the SWAPs between layers $L_{x}$ and $L_{x+1}$, the $A^{\ast}$ algorithm starts searching from the mapping of $L_{x}$, which we call $\sigma_{0}$. From $\sigma_{0}$, the algorithm tries to insert concurrent SWAPS, and it will produce successor mappings from different number of SWAPs. If for current mapping, it can only insert $n$ concurrent SWAPs at most. The successors would be the resulting successors of 1 SWAP, 2 SWAPs and so on till n SWAPs. All these successors would be ranked based on their cost (by putting into a priority queue), which is based on inherent cost and heuristic cost. If there are successors that fulfils the CNOT constraint of the following layer $L_{x+1}$, the search is ended and the CNOT-compliant successor with the least cost would be returned. If there are no CNOT-compliant successors, the search continues and the successor with least cost is spanned such that all its successors are added to the priority queue. The algorithm keeps the process until one CNOT-compliant successor is returned. 

\subsection{Choose the SWAP layer based on critical path}
This sections talks about how we make the algorithm more depth-aware. For the $A_{\ast}$ searching, it can find more than one CNOT-compliant mapping. We then evaluate all these CNOT-compliant candidates by adding it into the current circuit and calculate the resulting depth. It turns out the one with the least cost based on the heuristic normally does not result into smallest depth. We then choose the candidate that has the smallest depth as the one CNOT-compliant successor and return it. Algorithm \ref{algo} shows the details of how it works.

\begin{figure}[!ht]
  \centering
  \includegraphics[width=1\linewidth]{figs/algo.png}
  \caption{Choose the SWAP layer based on critical path}
  \label{fig:algo}
\end{figure}

\begin{algorithm}[h!t]
\label{algo}
\SetAlgoLined
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Input{Good Mapping Candidate G }
\Output{Best Mapping with the Least Circuit Depth}
\BlankLine

 best\_mapping = $\varnothing$\;
 critical\_path\_of\_best\_mapping = $\infty$\;
 \For{x $\in$ G}{
    new\_circuit = construct\_new\_circuit(original\_circuit, x)\;
    temp\_cp = calculate\_critical\_path(new\_circuit)\;
    \If{temp\_cp $<$ critical\_path\_of\_best\_mapping }{
        critical\_path\_of\_best\_mapping = temp\_cp\;
        best\_mapping = x\;
    }
 }
 
 \caption{Depth-aware SWAP Insertion}
\end{algorithm}



\subsection{Optimizations}

\subsection{Sensitivity Study}
\begin{figure}[htb]
  \centering
  \includegraphics[width=1\linewidth]{figs/sensitivity.png}
  \caption{Sensitivity to parameters}
  \label{fig:sensitivity}
\end{figure}
We use two parameters to tune our experiment: one is denoted as "expand" which means the number of nodes to expand at the each step of the search, and another one is denoted as "deeper" which means the number of deeper levels to go down after the search found the first CNOT-compliant mapping. These two parameters can go from 1 to larger numbers. By tuning these two parameters, we gradually yield the best results for our benchmarks. As we can see in Fig. \ref{fig:sensitivity}, with increasing these two parameters, there are more benchmarks achieve better performances. This shows that if we expand more nodes in the search and increase the search depth, there could be more better solutions found. It tells us that current heuristic-based qubit mapping solutions are still far from being optimal. 

==> slackq - arxiv/conclusion.tex <==
\section{conclusion}
The physical layout of contemporary quantum devices imposes limitations for
mapping a high level quantum program to the hardware. It is critical to develop
an efficient qubit mapper in the NISQ era. Existing
studies aim to reduce the gate count but are oblivious to the depth of the
transformed circuit. This paper presents the design of the
first time-efficient slack-aware swap insertion scheme. Experiment results show that our proposed solution generates hardware-compliant circuits with faster execution time
compared with state-of-the-art mapping schemes.
%, with negligible overhead of increased gate count. 



==> slackq - arxiv/evaluation.tex <==

\section{Evaluation}
\label{sec:eval}
In this section, we evaluate our  slack-aware swap insertion scheme (\textbf{SlackQ}) and compare it with the two state-of-the-art qubit mappers, respectively by \cite{Zulehner+:DATE18} and \cite{Li+:ASPLOS19}.  

\subsection{Experiment Setup}

    {\textbf{Benchmark.}} We use 106 benchmarks from RevLib~\cite{Wille+:ISMVL08}, IBM Qiskit \cite{IBMQiskit}, and ScaffCC \cite{JavadiAbhari+:CCF14}. RevLib comprises of a collection of benchmarks in the domain of reversible and quantum circuit design. Qiskit is a programming framework for quantum computing provided by IBM. ScaffCC is a compilation framework for the Scaffold quantum programming language. These benchmarks feature functionalities from implementing ALU logics, comparing inputs with constant values, ternary counters, to classic quantum algorithms like Quantum Fourier Transform (QFT) and ising model. 
    
     \noindent  {\textbf{Baseline}} We compare our work with two best known qubit
mapping solutions ~\cite{Zulehner+:DATE18}
(denoted as \emph{Zulehner}) and the Sabre qubit mapper from~\cite{Li+:ASPLOS19}
(denoted as \emph{Sabre}). We also compare our results with IBM's stochastic mapper in Qiskit \cite{IBMQiskit}. Since IBM's Qiskit mapper is significantly
worse in terms of circuit time than all other mappers we have evaluated, we do not show the results. The performance of Qiskit mapper is also noted in the work by \cite{Zulehner+:DATE18}.

    \noindent {\textbf{Metrics}} We compare the execution time of the transformed circuits generated by different qubit mapping strategies. It is worth mentioning that our approach can take any gate latency as input parameters and generate transformed circuits based on the input. However, to make evaluation results as close to real machines as possible, we use the results from the studies by \cite{murali+:asplos19, linke+:nas2017}. In these studies, different types of quantum architecture are investigated, and the studies reveal that two-qubit gates usually takes around twice as much time as single-qubit gates. Hence we assume single-qubit gates take 1 cycle and two-qubit CNOT gates take 2 cycles in our experiments. The time is reported as the total number of executed cycles.  


  \noindent {\textbf{Platform}} We use IBM's 20-qubit Q20 Tokyo architecture \cite{Li+:ASPLOS19} as the underlying quantum hardware. The qubit mapping approach is implemented in C++ and  executed on a Intel 2.4 GHz Core i5 machine, with 8 GB 1600 MHz DDR3 memory. 

\subsection{Experiment Analysis}

We categorize the 106 benchmarks into four categories. Benchmarks in the first category each has less than 200 gates, and we denote them as \textsf{mini} benchmarks. There are 22 mini benchmarks. The second category has benchmarks with 200 to 1,000 gates. We name this category as \textsf{small} benchmarks. There are 39 small benchmarks. The third category of benchmarks have 1,000 to 10,000 gates. We name it as \textsf{medium} benchmarks and there are 21 benchmarks in this category. The fourth category of benchmarks have 10,000 to 200,000 gates. We refer to it as \textsf{large} benchmarks and there are 24 benchmarks in this category. The results for \textsf{mini}, \textsf{small}, \textsf{medium}, and \textsf{large} benchmarks are presented in Fig. \ref{fig:mini_bench}, Fig. \ref{fig:small_bench}, Fig. \ref{fig:medium_bench}, and Fig. \ref{fig:large_bench} respectively. 

\begin{figure}[!ht]
  \centering
  \includegraphics[width=0.8\linewidth]{figs/small_speedup.pdf}
  \caption{Speedup for Mini Benchmarks (< 200 gates)}
  \label{fig:mini_bench}
\end{figure}


\begin{figure}[!ht]
  \centering
  \includegraphics[width=0.8\linewidth]{figs/medium_speedup.pdf}
  \caption{Speedup for Small Benchmarks (< 1000 gates)}
  \label{fig:small_bench}
\end{figure}

\begin{figure}[!ht]
  \centering
  \includegraphics[width=0.8\linewidth]{figs/large_speedup.pdf}
  \caption{Speedup for Medium Benchmarks (< 10000 gates)}
  \label{fig:medium_bench}
\end{figure}


\begin{figure}[!ht]
  \centering
  \includegraphics[width=0.8\linewidth]{figs/extra_large_speedup.pdf}
  \caption{Speedup for Large Benchmarks (< 200000 gates)}
  \label{fig:large_bench}
\end{figure}

It can be observed from the results that as the problem size scales, the performance improvement brought by \textsf{SlackQ} improves. For most benchmarks in the mini and small category, the speedup is between 1.1X and 1.5X. However, for the medium and large category, the speedup for most benchmarks is above or around 1.5X. The average speedup for mini benchmarks is 1.45X and for small, medium, and large benchmarks, the average speedup becomes 1.55X, 1.70X, and 1.86X respectively. The results show that our approach works well in general, and in particular for larger benchmarks.

There are two baselines we compare against: the Zulehner approach and the Sabre approach. For mini and small benchmarks, the \textsf{Zulehner} approach does not seem to perform as well as the \textsf{Sabre} approach. It can be seen from the fact that the relative speedup of \textsf{SlackQ} over \textsf{Zulehner} is usually larger than \textsf{SlackQ} over \textsf{Sabre}. However, the Sabre approach performs worse than the Zulehner approach for medium and large benchmarks. It can be seen that \textsf{Zulehner} and \textsf{Sabre} perform well in different scenarios when compared against each other. Regardless, our approach \textsf{SlackQ} outperforms both of them. 



==> slackq - arxiv/implementation.tex <==
\section{Implementation}

\label{sec:implemeatation}
Based on the design consideration on Section \ref{sec:insight}, we implement a slack-aware qubit mapping framework called \textsf{SlackQ}. 

\subsection{Overview of \textsf{SlackQ} }
Our algorithm is an iterative gate scheduler which dynamically resolves the connectivity issues encountered during the scheduling process. Initially, a dependency graph of the circuit is built. Then we traverse the dependency graph of the circuit and schedule the gates one by one. We keep a frontier set of gates ready to be scheduled.   
 When resolving the connectivity issues, we invoke a priority-queue based searcher for swap candidates. It returns hardware-compliant candidates.  
%sorted with respect to the number of swaps in ascending order. 
 Among these hardware-compliant candidates, the one that has the best slack utilization is  chosen, and the scheduling process proceeds.
 We describe the algorithm below with respect to the pseudo-code shown in Algorithm \ref{algo:search}:

\noindent \textbf{Step One - Initialization} This step prepares for the searching process. It builds the dependency graph of circuit. It finds the gates that do not depend on any other gates. Then it places those gates into the frontier $F$. It also initializes the processed gate set $P$ as empty set, and the remaining gate sets $R$ as the entire circuit. 

\noindent {\textbf{Step Two - Schedule Ready Gates}} This step goes through frontier list $F$. It finds all gates in $F$ that can be scheduled immediately due to having no connectivity issues according to the current mapping $\pi$. It schedules all these gates. When finishing the scheduling of one gate, it finds the descendant gate and see if this  descendant's other parent has also been scheduled. If this is the case, the descendant gate's dependency is resolved. It then places this descendant gate into $F$. This step is repeated until $F$ contains no gate that can be scheduled with respect to the current qubit mapping.

\noindent {\textbf{Step Three - Resolve Qubit Mapping Conflicts}} We go through the frontier $F$ again, finding the gates with resolved dependencies but are constrained by the current mapping and are on the critical path of the remaining circuit. Put those gates into a set called $F_{critical}$. Run a priority queue based searcher for hardware-compliant mappings. Our mapping searcher here returns a list of hardware-compliant mappings candidates, called $M$. 
%These returned mapping candidates are sorted with respect to gate counts in ascending order. 
Among these candidates, it finds the one (call it $m$) with the best slack utilization. Then we use the swap sequence associated with $m$ to update the mapping $\pi$ and add the swap sequence into the processed circuit P. % Update the dependency graph with added swaps from $m$.

\noindent {\textbf{Step Four}} Repeat Step Two and Three until all gates are scheduled in the circuit. Return transformed circuit. 

In Sections \ref{sec:impl_init} to \ref{sec:impl_resolve_conf}, we describe a few important aspects of this algorithm.
\vspace{-10pt}
\subsection{Initialization}
\label{sec:impl_init}
Before calling the scheduler described in Algorithm \ref{algo:search}, we initialize the frontier $F$ and processed circuit P, and the remaining circuit R. Initially, P is empty and R is the entire circuit. For $F$, it creates a Directed Acyclic Graph~(DAG) to represent the dependency between quantum operations.  Fig. \ref{fig:update_graph} (a) shows an example of a dependency graph from the circuit illustrated in Fig. \ref{fig:motivation} (b).  

%\begin{figure}[!ht]
%  \centering
%  \includegraphics[width=0.95\linewidth]{figs/DAG.pdf}
%  \caption{(a) The original circuit. (b) Generated DAG of the circuit. Red dashed rectangle denotes the frontier set $F$ at the beginning of the algorithm.}
%  \label{fig:dag}
%\end{figure} 

%A frontier set represents the set of gates whose dependency have been resolved. 
%The initial frontier set $F$ encloses the set of nodes with 0 in-degrees in the dependency graph. In Fig. \ref{fig:dag} (b) the initial frontier set is denoted in the red dashed rectangle. 

{\small
\begin{algorithm}[htb!]
\SetAlgoLined
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Input{Frontier $F$, initial mapping $\pi$, processed circuit $P$, remaining circuit $R$}
\Output{Transformed circuit T}
\BlankLine

\While{F not empty}{
    E = getSchedulableGates(F, $\pi$)\;
    \While{E not empty}{
        F.remove(E)\;
        P.add(E)\;
        R.remove(E)\;
        \For{g $\in$ E}{
            \For{d $\in$ g.children}{
                \If{d's dependency is resolved}{
                    F.add(d)\;
                }
            }
        }
        E = getSchedulableGates(F, $\pi$)\;
    }
    $F_{critical}$ = select\_critical\_gates ($F$)\;
    mapping\_candidates = resolve\_conflicts ($F_{critical}$, $\pi$)\;
    m = best\_slack\_utilization (mapping\_candidates, P, R)\;
    $\pi$  = update\_mapping\_with\_swaps(m, $\pi$)\;
    P.add(m.swaps)\;
}
return P\;
\caption{Dynamic Gate Scheduler} 
\label{algo:search}
\end{algorithm}
}

\vspace{-7pt}
\subsection{Choosing the Best Mapping Candidate}
With multiple hardware-compliant mappings, it is necessary to determine the candidate that has the best slack utilization. The best slack utilization means the inserted swap sequence makes best use of the slack currently existing in the circuit.
%, to minimize its impact on end-to-end circuit time. 
To evaluate these mapping candidates, for each of them, we tentatively insert the associated swap sequence and monitor how the swap insertions affect the dependence graph and the critical path. We trace the nodes that are affected due to the inserted swaps and detect how much their start/ending time changes. 

\begin{figure*}[!ht]
  \centering
  \includegraphics[width=0.95\linewidth]{figs/update_graph.pdf}
  \caption{(a) The generated dependency graph from the example of Fig. \ref{fig:motivation}. The numbers displayed on each gate refer to the start/end cycle of this gate.   (b) One mapping candidate whose inserted swap results in two later gates delaying its start/end cycles. (C) Another mapping candidate whose inserted swap does not affect the start/end cycles of the entire circuit.}
  \label{fig:update_graph}
\end{figure*} 

We again use the example circuit and qubit coupling graph in Fig. \ref{fig:motivation} to show how our evaluation approach works. We first show the original dependency graph in Fig. \ref{fig:update_graph} (a). The numbers on gates denote the start/end cycle of each gate. For instance, \textsf{[0, 1]} represents the start cycle as 0 and the ending cycle as 1. We assign a dummy gate node at the beginning of the circuit for each qubit $q1$ \char`\~ ~$q5$, for the sake of illustration. The dummy node starts at time 0 and takes 0 cycles. In this example, we have two possible mapping candidates whose swap sequences are to be inserted on different qubits. We need to choose the better one out of the two mapping candidates. The first mapping candidate shown in Fig. \ref{fig:update_graph} (b) inserts one swap on logical qubits $q2$ (the qubit for $g4$) and  $q3$ in between gates $g4$ and $g5$, corresponding to the circuit in Fig. \ref{fig:motivation} (d). It affects gates $g5$ and $g6$, which are marked in red. For each affected node in the dependence graph, to calculate its earliest start time, one needs to check each of its parent nodes' ending time, choose the maximum one, and use it as its own start time. In this example, added swap result in change in g5's start time as well as the change in g6'start time, and delays the entire circuit by 3 cycles. Here we assume each gate takes one cycle. We assume a swap is implemented using 3 CNOT gates and thus is 3 cycles. 
%in later gates having to delay their start cycles. 

The second mapping candidate shown in Fig. \ref{fig:update_graph} (c) inserts one swap on logical qubits $q3$ and $q5$ placed right in front of $g5$. It results in no changes to the start/end cycles of the entire circuit, since there is slack on physical qubits $q3$ and $q5$. Obviously, it should choose the mapping candidate illustrated in Fig. \ref{fig:update_graph} (c). 

We use an algorithm to systematically analyze the start/ending time of each gate due to inserted swaps. The algorithm does not have to traverse the entire dependence graph. Instead, it only traces the affected gates in the original circuit to find the candidate that leads to the smallest increment to total circuit time. We also add an optimization to quickly terminate the tracing when a candidate is deemed hopeless. A candidate is deemed hopeless if one of the affected gates is on the critical path and the delay to that gate due to swaps already exceeds the smallest increment found in a previous candidate. In that case, it terminates the tracing and moves on to the next candidate. 
%for checking nodes in the critical path of the circuit before inserting the swap gates. If at one point of checking the affected nodes in the DAG corresponding to one mapping candidate, a gate on the critical path is already delayed by more than the minimal increased execution time for all previous checked mapping candidates, there is no need to continue checking the rest of the nodes of the DAG for the current mapping candidate.  At this point, the algorithm can move on to check other mapping candidates. 
The algorithm is described in Algorithm \ref{algo:update_graph}. 


{\small
\begin{algorithm}[htb!]
\SetAlgoLined
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Input{Mapping candidates $M$, dependency graph $G$, proessed circuit $P$}
\Output{Best slack-utilizing mapping $m_{best}$}
%\BlankLine
smallest\_inc = $\infty$\;
CP = getCriticalPath(G)\;
\For{$m \in M $}{
    $RG$ = getLastScheduledGateOnEachQubit(P)\;
    G' = G\;
    G'.addGates(m.swaps)\;
    graph\_updated = True\;
    circuit\_time = 0\;
    \While{$RG$ not empty}{
        $RG'$ = []\;
        \For{$g \in RG$}{
            g.updateTentativeStartAndEndCycle()\;
            delta = g.tentativeStart - g.originalStart\;
            \If{g is on critical path \& delta > smallest\_inc}{
                graph\_updated = False\;
                break the while loop\;
                
            }
            \If{delta > 0}{
                RG'.add(g.children)\;
            }
            circuit\_time = max(circuit\_time, g.tentativeEnd)\;
        }
        RG = RG'\;
    }
    \If{(graph\_updated == True \& circuit\_time $>$ CP)}{
        %inc = circuit\_time - CP\;
        \If{ ( (circuit\_time - CP) $<$ smallest\_inc )} {
        smallest\_inc = circuit\_time - CP \;
        $m_{best}$ = m\;}
    }
}
return $m_{best}$\;

\caption{Find the best slack-utilizing mapping} 
\label{algo:update_graph}
\end{algorithm}
}

\vspace{-10pt}
\subsection{Navigating the Candidate Search Space}
\label{sec:impl_resolve_conf}
We use a priority queue based searcher for qubit mapping candidates. The search space consists of state nodes that represent possible mappings from logical qubits to physical qubits. A mapping can be represented as $\pi: \{q_{1}, q{2}, ..., q_{n}\} \to  \{Q_{1}, Q{2}, ..., Q_{n}\}$. Applying swaps on top of a mapping can convert it into another mapping. Specifically, if we apply "$swap$ $q_{i}, q_{j}$" on a certain mapping $\pi_{old}$  and create the resulting mapping $\pi_{new}$, we will have $\pi_{new}[q_{i}] = \pi_{old}[q_{j}]$ and $\pi_{new}[q_{j}] = \pi_{old}[q_{i}]$. 


Given $F_{critical}$ and current mapping $\pi$, it starts searching the state space of all feasible mappings that satisfy $F_{critical}$. It picks a node to expand and enumerate all possible parallel one-step swaps as the node's successors. We use a priority queue that is similar to that in \cite{Zulehner+:DATE18}. Unlike the work by \cite{Zulehner+:DATE18} where the search stops when the first state node that resolves all connectivity conflicts is retrieve from the priority queue, our search stops after $m$ expansions since the mapping candidate with minimal swap count is found, or when the gate count of the mapping candidate that is just retrieve has less than or equal to $k$ times more gates than the minimal swap count. We set $m=20$ and $k=2$ such that the returned mapping candidate will have reasonable gate counts. After all mapping candidates have been retrieved, we rank them with respect to the metric of best slack utilization discussed above. 


%The priority queue based search returns a set of hardware-compliant mappings for which the gate count is bounded with respect to the minimal gate count by $k$ times. 

%It will expand the state node of $\pi$ by doing the following: It enumerates all possible one concurrent swap, two concurrent swaps, three concurrent swaps, all the wap up to $n/2$ concurrent swaps, where $n$ is the number of qubits in the circuit; Each set of concurrent swaps lead to a new mapping, and the new mapping becomes a child of $\pi$. The total number of successors of $\pi$ is up to ${n \choose 1}$ + ${n \choose 2}$ + ... + ${n \choose n}$. 
%In this process, we only keep the nodes that at least have a swap that involves a logical qubit in $F_{critical}$ to prune the search space. All newly generated successors will be checked to see if it resolves qubit mapping conflicts in $F_{critical}$. Each successor of $\pi$ can be further expanded in the same way. The search goes on until it finds a set of state nodes which meets our criteria. The state nodes would have the mapping that solves all conflicts. Exhaustive search in this space is prohibitive. We use a priority queue to guide the expanding of nodes in the frontier of the search tree. The nodes that need to be expanded are placed into the priority queue with respect to a cost function $f(x) = g(x) + h(x)$, with $g(x)$ representing the cost of the path from root node to $x$ and $h(x)$ representing the estimate cost from $x$ to target node. In our implementation, $g(x)$ is the number of swaps that have already incurred for state node $x$. The $h(x)$ estimates at least how many more swaps are still needed, which is approximated as the shortest physical distance of the qubits for at least one CNOT that is in the $F_{critical}$ set and hasn't be resolved. The heuristic function is similar to a classical A-star algorithm. Unlike A-star, our algorithm does not terminate when the mapping candidate with minimal cost function is achieve when d, i.e., when the mapping candidate with minimal swap gate count is achieved. Instead, we continue the search and keep expanding nodes from the priority queue up to a certain point when we have enough feasible mapping candidates. The output will be a list mapping candidates sorted with respect to the swap gate count in ascending order. 

 


==> slackq - arxiv/insight.tex <==
\section{Insight and Design}
\label{sec:insight}
To improve the parallelism between the inserted SWAP operation and the gates in the original circuit, we discover that it is important to exploit the \textsf{slack} intervals in the circuit. The slack represents the idle time in the original circuit for a given set of qubits. The key is to hide the latency of inserted swap operations by using the qubits that are idle at that time of the circuit execution. This forms the main idea of this paper and we insert SWAP operations such that they leverage \textsf{slack} in the circuit as much as possible.
%hide the latency of inserted swaps as much as possible. 

\subsection{Slack}
\label{sec:slack}
We define \textsf{slack} as the idle time between two consecutive gates on the same qubit(s) and can be used to perform SWAP operation without affecting the total execution time of the entire circuit. The \textsf{slack} time is usually caused by dependence between gates and/or variation of gate count on individual qubits.

The \textsf{slack} time due to dependence between gates only occurs when there are two-qubit gates in the circuit. Recall that a CNOT gate depends on up to two other gates, since CNOT is a two-qubit gate. If the qubits are running at different speeds, one of the other qubits might be ready earlier than the other. The faster qubit thus needs to wait for the slow qubit to finish before the CNOT gate can be executed. On the other hand, if a circuit has a number of qubits, and the number of gates on each qubit is different (even if they are all independent), then some qubits will inevitably be idle at some point of the execution. The slack intervals can be used for inserting swap operations that resolve qubit mapping constraints. An example of \textsf{slack} in the circuit is shown in Fig. \ref{fig:slack_cycles}. 

%qubits that gate that depends on two other gates,  If one CNOT gate depends on two other gates  in a \fixit{You may talk about the reasons that cause a slack} 

\begin{figure}[h]
  \centering
  \includegraphics[width=0.75\linewidth]{figs/slack_example.pdf}
  \caption{Slack in the circuit: Since \textsf{g3} depends on \textsf{g1} and \textsf{g2}, \textsf{g1} finishes earlier than g2, therefore, for qubit \textsf{q3}, there is a slack interval of three cycles (assuming each gate takes one cycle) between \textsf{g1} and \textsf{g3} in the circuit. }
  \label{fig:slack_cycles}
\end{figure}



\begin{figure*}[htb]
  \centering
  \includegraphics[width=0.9\linewidth]{figs/frainsight.pdf}
  \caption{(a) Qubit coupling graph; (b) An example of fixed slack in the quantum circuit; (c) and (d) Examples of flexible slacks, where \textsf{g1} can be moved within a time window without affecting the circuit execution time, the slack before g1 can be either 1 cycle or 2 cycles assuming every gate takes one cycle. Note the slack between \textsf{g1} and \textsf{g3} may also vary due to scheduling of g1. }
  \label{fig:remainingcircuit}
\end{figure*} 

There are two types of slacks in the circuit. One type does not require the rescheduling of the gates, and we define it as \textsf{fixed slack}. The other type of slacks may have variable number of cycles, and we denote it as \textsf{flexible slack}. A good qubit mapper needs to search globally and exploit both \textsf{fixed} and \textsf{flexible slack}.

\vspace{-5pt}
\paragraph{\textbf{Fixed Slack}} An example of \textsf{fixed slack} is shown in Fig. \ref{fig:remainingcircuit} (b). Assuming each gate takes one cycle, there is a fixed slack between \textsf{g1} and \textsf{g2} on qubit \textsf{q2}. Here it cannot delay g2 or start g1 early if the total execution time needs to remain unchanged. If qubit \textsf{q2} is used to perform another gate such as the swap operation during the three cycles, it will not affect the execution time of the entire circuit. In this case, the number of cycles that can be used on \textsf{q2} between g1 and g2 is fixed. 

\begin{figure}[!ht]
  \centering
  \includegraphics[width=1.0\linewidth]{figs/fraidea.pdf}
  \caption{Choose SWAP Candidates}
  \label{fig:algo}
\end{figure}

\vspace{-10pt}
\paragraph{\textbf{Flexible Slack}} Sometimes fixed slack does not always exist. It is necessary to move the gates in order to create slacks for latency hiding purpose. We show an example Fig. \ref{fig:remainingcircuit} (c) and (d), where slack can be created by moving $g1$. Let's say cnot($q{1}, q{2}$) and cnot($q_{3}, q_{4}$) are scheduled on cycle 1. The three single-qubit gates on $Q_{1}$ are scheduled on cycle 2,3,4 respectively. With this going on, $g{3}$ expects to be executed on cycle 5 at the earliest. $g{3}$ depends on $g{1}$. $g{1}$ can be scheduled at the second cycle, the third cycle (Fig. \ref{fig:remainingcircuit} (c) ) or the fourth cycle (Fig. \ref{fig:remainingcircuit}  (d)) without delaying $g5$. To this end, a slack with zero, one or two cycles can be created between $g2$ and $g1$, depending on when $g1$ is scheduled. And this type of slack between $g2$ and $g1$ is flexible. On the other hand, since $g1$ is not directly executable due to the connectivity constraint in Fig. \ref{fig:remainingcircuit} (a), the more slack intervals before $g1$ there are, the better it is for hiding the swap latency. In Fig. \ref{fig:flexibleslack}, we show that by moving $g{1}$ forward, q2 and q3 can have more slack intervals before $g1$, and swap(3,4) is inserted which utilizes the slack, resulting in a total circuit time of 6 cycles only, which is optimal in this case. 

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{figs/framework_example.pdf}
    \caption{Scheduling gates to create more slacks: gate \textsf{g1} can be moved forward such that \textsf{swap Q3, Q4} can absorb the longer slack on q3}
    \label{fig:flexibleslack}
\end{figure}

It is worth mentioning flexible slack could be cascading as the rescheduling of one gate might affect its descendants or predecessors. For the fixed slack, the gates involved cannot be delayed without affecting the circuit time. Flexible slack allows one or multiple gates to delay start within reasonable time window(s). Flexible slack are more complicated than fixed slack. It is necessary to analyze and exploit flexible slack in a systematic way.  


\vspace{-5pt}
\subsection{Dynamic Gate Scheduler}
We model the resolution of qubit mapping conflicts as a dynamic scheduling process. Gates in the circuit are scheduled as soon as their dependencies are resolved. When a gate cannot be scheduled due to a connectivity problem, we insert a (combination of) swap(s) to change the qubit mapping so that the gate can be executed on the physical device. All the gates that have already been scheduled at one point of scheduling are called the \textsf{Processed Circuit}, and the gates that still await scheduling are called the \textsf{Remaining Circuit}. 

\begin{figure*}[!ht]
  \centering
  \includegraphics[width=1\linewidth]{figs/criticality.pdf}
  \caption{(a) Qubit Connectivity for a five-qubit machine (b) Original Circuit before qubit mapping (c) \textbf{Strategy One:} Resolving gates on critical path first (d) \textbf{Strategy Two:} Resolving gates on non-critical path first. }
  \label{fig:criticality}
\end{figure*}

Fig. \ref{fig:flexibleslack} shows an example of how the scheduling works. With initial mapping of $\{q_{1}, q_{2}, q_{3}, q_{4}\} \to \{Q_{1}, Q_{2}, Q_{3}, Q_{4}\}$, the first two CNOTs \textsf{cnot($q_{1}, q_{2}$)} and \textsf{cnot($q_{3}, q_{4}$)} and the three single-qubit gates on $Q{1}$ can be scheduled without remapping. At this point, those gates that are scheduled are part of the \textsf{Processed Circuit}. The remaining two CNOT gates ($g{1}$ and $g3$) that cannot be scheduled are part of the \textsf{Remaining Circuit}. Gate $g{1}$ cannot be scheduled because Q2 and Q3 are not connected in the device. Gate $g{3}$ cannot be scheduled because $g{1}$ must be scheduled before $g{3}$ (write-after-read dependency on Q2). The dashed lines divide the circuit into processed part and remaining part. 

To minimize the circuit time, we search for swap candidates for $g{1}$ that results in maximally hiding swap latencies using circuit slack. Fig. \ref{fig:algo} shows the key idea behind the searching for optimal swap candidates. The search reveals multiple hardware-compliant candidates that utilize different sequences of swaps to achieve compliance.  We choose the optimal candidate by calculating the \emph{Slack Utilization} of each candidate, and choosing the one with the best utilization. In Fig. \ref{fig:flexibleslack}, we choose swap candidate \textsf{swap(q3, q4)} since it best hides the swap latency behind the 2-cycle slack shown in Fig. \ref{fig:remainingcircuit} (d). Now $g{1}$ is satisfied and scheduling can proceed. 

%This is how we analyze all potential swap candidates, and find the one that minimizes the increment to the entire circuit time. 




\subsection{Critical Gates}
The gates in the remaining circuit  pending scheduling whose dependences have been resolved but connectivity problems haven't been can be divided into two groups: those on the critical path and those that are not. We denote the gates on the critical path as \textsf{critical gates}, and the others as \textsf{non-critical gates}. In parallel computing, the critical path length is equal to the execution time when there is enough parallelism. In this case, the critical path is equal to execution time as the maximum parallelism (the maximum number of gates that can run concurrently) is at most the same as the number of qubits. Thus it is important to prioritize the scheduling of critical gates over non-critical gates. 
% and hence to resolve conflicts of critical path over that of normal gates. 

To prioritize critical gates, what we need to do is to resolve the connectivity problems of critical gates as early as possible. Imagine a scenario where two gates have connectivity problems, one gate is critical and the other is non-critical gate. Their connectivity issues cannot be resolved at the same time. Under this situation, we should resolve the critical gate first, as resolving the \textsf{non-critical} gates can be likely delayed without affecting the overall execution time. 
 
 


We use an example from Fig. \ref{fig:criticality} to show how \textsf{criticality} can play an important role in determining the overall circuit time. We use a five-qubit quantum machine, whose connectivity is shown in Fig. \ref{fig:criticality} (a). This example circuit consists of 4 CNOTs and 3 single-qubit gates, with $g{1}$, $g{2}$ scheduled, and $g{3}$, $g{4}$ not yet scheduled due to connectivity issues. It's crucial to note that $g_{3}$ is on the critical path, while $g{4}$ is not. The two gates $g{3}$ and $g{4}$ cannot be resolved at the same time if both of them want to use only one swap, since qubit $C$ is the on the path from $T1$ to $T2$, and from $X1$ to $X2$. Whether to prioritize $g{3}$ over $g{4}$ when using the hub qubit $C$ for swap, makes a big difference in terms of circuit time. We show this discrepancy by illustrating two strategies and their resulting circuits. 
\begin{itemize}
\item {\textbf{Strategy One - Prioritizing critical gates}}  Resolve $g{3}$ first. Shown in Fig \ref{fig:criticality} (c), it is necessary to insert swap($q2$, $q3$) before $g{3}$. After $g{3}$ is resolved and scheduled, swap($q2$, $q4$) is inserted such that $g{4}$ can be resolved. swap($q2$, $q4$) can take advantage of the slack on logical qubits $q2$ and $q4$, as logical qubit $q1$ is processing three single-qubit gates. This strategy results in total circuit time of 10 cycles, assuming CNOT and single-qubit gate both have latencies of one cycle.

\item {\textbf{Strategy Two - Not distinguishing  critical gates from non-critical path}} Resolve $g{4}$ first. Shown in Fig \ref{fig:criticality} (d), it is necessary to insert swap($q3$, $q4$) before $g{4}$, and let $g{4}$ be scheduled. In the meantime, $g{3}$ has to wait, which results in the critical path being elongated due to the delay of the execution time of $g{4}$ and swap($q3$, $q4$).  It is because when $g{4}$ is being executed, the mapping that allows $g{4}$ must be kept, which will delay all the remaining gates. In this case, it is not desirable to delay all the remaining gates as they are on critical path. Delaying gates that are  critical will have a more detrimental impact than delaying gates not on critical path. After $g{4}$ is resolved, the fastest way to resolve $g{3}$ is to swap($q2$, $q4$) before $g{3}$. This strategy as a whole results in total circuit time of 13 cycles, which is 30\% more than strategy one. 
\end{itemize}

It can be seen from this example the later resolving of the non-critical gates are highly likely to overlap with the gates on the critical path, and result in less impact to overall circuit execution.


%It clear shows that by prioritizing critical gate $g_{3}$ over normal gate $g_{4}$, we are able to save the circuit time by 23\% (3/13). 

==> slackq - arxiv/propose.tex <==
\section{Insight and Design}

\subsection{Metric}
As our work is a depth-aware SWAP insertion scheme, we first precisely define the metric for characterizing the depth of a circuit. In order to fully explain the metric, we need to introduce the concepts of \emph{dependency graph} and \emph{critical path}. 

The dependency graph represents the precedence relation between quantum gates in a logical quantum circuit. The definition is below:

\begin{definition}{Dependency Graph} :
The dependency graph of a quantum circuit $C$ with a set of gates $\Psi$ is a Directed Acyclic Graph $G_\psi=(\Psi, E_\psi)$, $E_\psi \subseteq \psi \times \psi$. A directed edge from node $\psi_1$ to node $\psi_2$ exists if and only if the output of gate $\psi_1$ is (part of) the input of gate $\psi_2$ in the quantum circuit $C$.
\end{definition}

The critical path is referred to as the longest path in the dependency graph. And the definition is below:


\begin{definition}{Critical Path} :
Given a dependency graph $G_\psi=(\Psi, E_\psi)$ of a quantum circuit. The critical path is $CP=Max(Path(\psi_1, \psi_2))$ $ s.t.$ $\psi_1, \psi_2 \in E_{\psi}$ $and$ $ \psi_1 \neq \psi_2$ 
\end{definition}


The depth is characterizing the number of execution steps of a quantum circuit, which is tantamount to the critical path length of the circuit. The longest path in the dependence graph describes the minimal number of steps the circuit needs in order for every gate's data dependence be resolved. In Algorithm \ref{algo}, we show how we calculate the critical path.
\begin{algorithm}[htb]
\label{algo}
\SetAlgoLined
\SetKwInOut{Input}{Input}
\SetKwInOut{Output}{Output}
\Input{The circuit's dependency graph $G(V,E)$ }
\Output{The critical path $CP$}
\BlankLine

%  best\_mapping = $\varnothing$\;
%  critical\_path\_of\_best\_mapping = $\infty$\;

 earliest\_start = \{\}\;
 CP = 0\;
 
 
 \For{n $\in$ V in topological order}{
    temp = 0\;
    \For{p $\in$ V's predecessors} {
      \If {temp $<$ earliest\_start[p] + latency[p]}{
         temp = earliest\_start[p] + latency[p]\;
      } 
    }
    earliest\_start[n] = temp\;
      \If {CP $<$ temp + latency[n]} {
         CP = temp\;
      }
 }
 
 
 
return CP \;
 
 \caption{Calculate the Critical Path of a Circuit}
\end{algorithm}


We first sort the nodes in the directed acyclic graph in topological order. Then we process the nodes in that order. For each node, we check the earliest start time for each of its predecessors, and add it by the latency of that predecessor, then we choose the maximum and use it as the earliest start time of this node. The maximum of all nodes' earliest start time added by their latency is the critical path length. 

We use the critical path length as the metric for ranking different swap insertion options.




% The circuit is comprised of quantum gates applied on qubits in a time order, which means a dependency tree for quantum gates can be built based on their order applied on each qubit. The critical path of this dependency tree is equal to the depth of the entire circuit. For adding SWAP into the circuit, if it's not on the critical path it is possible the result depth would not be increased. A clear example is shown in Fig. \ref{fig:simple_exp} (d), where the inserted two SWAPs render no depth increase to the circuit. In this sense, the added SWAPs overlap 100\% with existing circuit. 

% A na\"ive way towards realizing the need to overlap with the circuit, is to maximally overlap the inserted SWAPs with the already processed part of the circuit. At the certain point of needing to insert SWAPs, what we have is the already processed part of the circuit, but the remaining is still untouched. It naturally leads to the goal of merging SWAPs with existing circuit. But normally the case is that there is actually not enough potential to overlap with the previous part of the circuit. This example here clearly shows that in Fig. \ref{fig:remainingcircuit}, there is also potential to explore in the remaining circuit.

% This marks our insight that, when choosing the candidates of a SWAP set, it's ideal to consider its potential to overlap with not the existing processed circuit but the entire circuit from beginning to the end.

\subsection{Framework Design}
With the metric precisely explained in previous section, now we continue to explain the work flow of our framework and the intuitions behind it.

Before delving into the details of this framework, we need to define the \emph{layer} and the \emph{coupling graph}.

\begin{figure}[htb]
  \centering
  \includegraphics[width=0.9\linewidth]{figs/framework.pdf}
  \caption{The Qubit Mapping Framework}
  \label{fig:workflow}
\end{figure} 


\begin{definition}{Coupling Graph} : 
The coupling graph of a quantum architecture $X$ with a set of physical qubits $Q$ is a directed graph $G=(Q, E)$, $E\subseteq Q\times Q$. The edge $E_{x}=(Q_1,Q_2)\in E$ if and only if a $CNOT$ gate can be applied to $Q_1$ and $Q_2$ in $X$ with $Q_1$ being the control qubit and $Q_2$ being the target qubit. 
\end{definition}

We can divide the set of quantum gates in a circuit into layers, so that all gates in the same layer can be executed concurrently. The formal definition of a layer is:

\begin{definition}{Layer} :
A quantum circuit $C$ can be divided into layers $L = 
{l_1,l_2,l_3,...,l_m}$, while $\bigcup_{i=1}^{m}l_i = C$ and $\bigcap_{i=1}^{m}l_i = \emptyset$. The set of gates at layer $l_i$ can run concurrently  and  act on distinct sets of qubits.
\end{definition}
To divide a circuit into layers, we group the gates that have the same \emph{earliest start time} (defined in Algorithm \ref{algo}) into the same layer. The order of the layers is thus determined by the order of the \emph{earliest start times}.   

We use an iterative process to find the mapping. Our framework is depicted in Fig. \ref{fig:workflow}. And this iterative process is explained as below.
We start the framework by taking the input of the coupling graph (also denoted as \emph{Qubit Connectivity}) and the original circuit's initial layer. 

We process the circuit layer by layer. Given a layer, we perform the following steps.
    \begin{itemize}
        \item We check the layer to see if it is hardware-compliant based on the coupling graph and the qubit mapping before current layer is scheduled.
        \item If YES, we move on to next layer.
        \item If NO, we invoke our mapping searcher to search for (the set of) swaps that are necessary to solve the current layer. We consider depth-awareness during the selection of the set of swap gates -- the resulted mapping of which generates the smallest critical path length (described in Section \ref{sec:map}). After we find a hardware-compliant mapping, we move to the next layer. 
    \end{itemize}
    
    After all layers are processed, the mapping terminates. 

\subsection{Circuit Mapping Searcher}
\label{sec:map}
Here we describe the specific mapping searcher we use to overcome the coupling constraint for a given layer. 

We build our method upon the 
\emph{A-star} algorithm for finding valid mappings that minimize the number of only the inserted SWAP gates \cite{Zulehner+:DATE18}. We extend it by changing the ranking metric and allowing it to search for feasible mappings that do not necessarily have the smallest SWAP gate counts. It will help us search in a way that minimizes the depth while not significantly increasing the gate count.


%To be depth-aware for the searching process, it is important how we take the focus of depth into consideration. Thus the goal of searching becomes to find the mapping that minimizes the resulting depth while also reducing increased gate count as few as possible. 

We rank the swap options by the increase in the critical path length. Since it is an iterative process that handles the gates layer by layer, it is tempting to consider only minimizing the depth of the already processed circuit when deciding which swaps to use.  

\begin{figure}[htb]
  \centering
  \includegraphics[width=0.9\linewidth]{figs/frainsight.pdf}
  \caption{(a) Layout of an example architecture with 4 physical qubits (b) Example of a quantum circuit, the dashed line separates the processed circuit and the remaining circuit (c) Inserted SWAP overlaps with remaining circuit instead of existing processed circuit}
  \label{fig:remainingcircuit}
\end{figure} 

But the example in Fig. \ref{fig:remainingcircuit} shows that not only the processed circuit, but also the remaining circuit can help overlap the SWAPs with existing gates in the circuit without affecting the critical path.  As shown in Fig. \ref{fig:remainingcircuit}, for the CNOT gate (in red), there is no way it can overlap the necessary SWAPs with the processed circuit (dubbed as the circuit before the dashed line). But when we look after the dashed line, the three single-qubit gates can overlap with inserted SWAP. And this renders less impact to the depth of the resulting circuit, compared to if we insert the SWAP on $Q_1$ and $Q_2$.

Based on this intuition, we design our scheme of choosing the SWAP candidate as in Fig. \ref{fig:algo}. For each of the hardware-compliant remapping candidates that we acquire from the \emph{A-star} searcher, we calculate the critical path after merging the candidate (set of) swap(s) with both the processed circuit and the not-processed circuit. We choose the mapping that yields the shortest critical path.

\begin{figure}[!ht]
  \centering
  \includegraphics[width=1\linewidth]{figs/fraidea.pdf}
  \caption{Choose SWAP Candidates}
  \label{fig:algo}
\end{figure}


% \begin{figure}[!ht]
%   \centering
%   \includegraphics[width=1\linewidth]{figs/astar.png}
%   \caption{Overview of the $A^{\ast}$ searching}
%   \label{fig:astar}
% \end{figure}

% As shown in Fig. \ref{fig:astar}, the $A^{\ast}$ algorithm starts searching from current mapping. From current, the algorithm tries to insert concurrent SWAPS, and it will produce successor mappings from different number of SWAPs. If for current mapping, it can only insert $n$ concurrent SWAPs at most. The successors would be the resulting successors of 1 SWAP, 2 SWAPs and so on till n SWAPs. All these successors would be ranked based on their cost (by putting into a priority queue), which is based on inherent cost and heuristic cost. If there are successors that fulfils the CNOT constraint of the following circuit, the search is ended and the CNOT-compliant successor with the least cost would be returned. If there are no CNOT-compliant successors, the search continues and the successor with least cost is spanned such that all its successors are added to the priority queue. The algorithm keeps the process until one CNOT-compliant successor is returned. 

\subsection{Optimizations}
% The search for SWAPs start from the current mapping that needs change. And during the search process in the $A^{\ast}$ algorithm, each node inside the search tree represents a temporary mapping. 

% For the $A^{\ast}$ searching, it can find more than one CNOT-compliant mapping. We then evaluate all these CNOT-compliant candidates by adding it into the current circuit and calculate the resulting depth. It turns out the one with the least cost based on the heuristic normally does not result into smallest depth. We then choose the candidate that has the smallest depth as the one CNOT-compliant successor and return it.


We use two ways to optimize our proposed solution. One is to expand more nodes during the \emph{A-star} search, and another one is to search into deeper levels.
\subsubsection{Expand More Nodes}
In the search process for \emph{A-star}, the normal routine is to expand the one node of least cost at each step. Here, we can expand more than one node at each step and increase the search space. The number of nodes that can be expanded at a time can go from 1 to larger number. 
%In our experiments, we choose to expand 5 at one step.  
\subsubsection{Deeper Search}
 We increase the depth of the A-star search tree. In normal case, the search process ends when it finds the first node that minimizes the number of SWAPs, which is reflected as a certain level of the A-star tree. To this end, the second optimization that we applied here is to continue the search into a deeper level of the A-star tree. We can specify and tune the parameter of the deeper search. %This number can be tuned. %and we set this parameter to 4 in this paper. 

By tuning these parameters, there are more possible nodes added into our search space. With a larger search space, we have a larger possibility to jump out of one local optima and go to the global optima.

